Density and Velocity Correlations in Isothermal Supersonic Turbulence

In star-forming clouds, high velocity flow gives rise to large fluctuations of density. In this work we explore the correlation between velocity magnitude (speed) and density. We develop an analytic formula for the joint probability distribution (PDF) of density and speed, and discuss its properties. In order to develop an accurate model for the joint PDF, we first develop improved models of the marginalized distributions of density and speed. We confront our results with a suite of 12 supersonic isothermal simulations with resolution of $1024^3$ cells in which the turbulence is driven by 3 different forcing modes (solenoidal, mixed and compressive) and 4 r.m.s. Mach numbers (1, 2, 4, 8). We show, that for transsonic turbulence, density and speed are correlated to a considerable degree and the simple assumption of independence fails to accurately describe their statistics. In the supersonic regime, the correlations tend to weaken with growing Mach number. Our new model of the joint and marginalized PDFs are a factor of 3 better than uncorrelated, and provides insight into this important process.

==> data_analysis.tex <==
\section{Data collection and analysis}

Treating frames as ensembles, averaging over frames...

A few very important notes about power trees (can we call the binary/quadtrees that?), creating PDF's in 1D and 2D, weighing (very important!). Volume weighing, mass weighing, energy weighing. Must be done before any PDFs are introduced to make any sense.

\subsection{Power trees}

Importance sampling according to the histogram itself, keeping the probability per bin roughly constant. Works in any D, hence power tree (binary tree, quadtree, octree).

==> mnras_toc.tex <==

% The MNRAS class isn't designed to include a table of contents, but for this document one is useful.
% I therefore have to do some kludging to make it work without masses of blank space.
\begingroup
\let\clearpage\relax
\tableofcontents
\endgroup
\newpage

